A Multiwavelength Survey of Nearby M dwarfs: Optical and Near-Ultraviolet Flares and Activity with Contemporaneous TESS, Kepler/K2, \textit{Swift}, and HST Observations

We present a comprehensive multiwavelength investigation into flares and activity in nearby M~dwarf stars. We leverage the most extensive contemporaneous dataset obtained through the Transiting Exoplanet Sky Survey (TESS), Kepler/K2, the Neil Gehrels Swift Observatory (\textit{Swift}), and the Hubble Space Telescope (HST), spanning the optical and near-ultraviolet (NUV) regimes. In total, we observed 213 NUV flares on 24 nearby M dwarfs, with $\sim$27\% of them having detected optical counterparts, and found that all optical flares had NUV counterparts. We explore NUV/optical energy fractionation in M dwarf flares. Our findings reveal a slight decrease in the ratio of optical to NUV energies with increasing NUV energies, a trend in agreement with prior investigations on G-K stars' flares at higher energies. Our analysis yields an average NUV fraction of flaring time for M0-M3 dwarfs of 2.1\%, while for M4-M6 dwarfs, it is 5\%. We present an empirical relationship between NUV and optical flare energies and compare to predictions from radiative-hydrodynamic and blackbody models. We conducted a comparison of the flare frequency distribution (FFDs) of NUV and optical flares, revealing the FFDs of both NUV and optical flares exhibit comparable slopes across all spectral subtypes. NUV flares on stars affect the atmospheric chemistry, the radiation environment, and the overall potential to sustain life on any exoplanets they host. We find that early and mid-M dwarfs (M0-M5) have the potential to generate NUV flares capable of initiating abiogenesis.

==> uv_flare_properties.tex <==
% \documentclass[twocolumn]{aastex631}
% \newcommand{\vdag}{(v)^\dagger}
% \newcommand\aastex{AAS\TeX}
% \newcommand\latex{La\TeX}
% \newcommand{\swift}{\textit{Swift}\xspace}

% \usepackage{longtable}

% \title{Summary of near UV flare properties}

% \begin{document}

\begin{longtable}{|l|l|l|l|l|l|l|l|l|l|}
\caption{Summary of NUV flare properties} \label{tab:long} \\

\hline \multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{$N_{U}$}} & \multicolumn{1}{c|}{\textbf{$N$}} & \multicolumn{1}{c|}{\textbf{$T_{\rm start}$}} & 
\multicolumn{1}{c|}{\textbf{$T_{\rm stop}$}} & \multicolumn{1}{c|}{\textbf{duration}} & 
\multicolumn{1}{c|}{\textbf{Peak Flux}}  & \multicolumn{1}{c|}{\textbf{amplitude}} & \multicolumn{1}{c|}{\textbf{energy}}
& \multicolumn{1}{c|}{\textbf{$L_{q}$}}\\
\hline  \multicolumn{1}{|c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{}}  & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & 
\multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & \multicolumn{1}{c|}{min} & 
\multicolumn{1}{c|}{cnts/s}  & \multicolumn{1}{c|}{\textbf{}}  & \multicolumn{1}{c|}{10$^{30}$ erg}
& \multicolumn{1}{c|}{erg s$^{-1}$}\\
\hline 
\endfirsthead

\multicolumn{10}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{$N_{U}$}} & \multicolumn{1}{c|}{\textbf{$N$}} & \multicolumn{1}{c|}{\textbf{$T_{\rm start}$}} & 
\multicolumn{1}{c|}{\textbf{$T_{\rm stop}$}} & \multicolumn{1}{c|}{\textbf{duration}} & 
\multicolumn{1}{c|}{\textbf{Peak Flux}}  & \multicolumn{1}{c|}{\textbf{amplitude}} & \multicolumn{1}{c|}{\textbf{energy}}
& \multicolumn{1}{c|}{\textbf{$L_{q}$}}\\ \hline 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & 
\multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & \multicolumn{1}{c|}{min} & 
\multicolumn{1}{c|}{cnts/s}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{10$^{30}$ erg}
& \multicolumn{1}{c|}{erg s$^{-1}$}\\
\hline
\endhead

\hline \multicolumn{10}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

AP Col & 10 & 1 & 1473.0841 & 1473.0869 & 4.2 & 25.4 & 39.1 & 3.8 & 27.4 \\
        &    & 2 & 1473.2044 & 1473.2063 & 2.9 & 2.4 & 3.7 & 0.33 & \\
        &   & 3 & 1482.0536 & 1482.0556 & 3.1 & 10.3 & 14.5 & 1.6 & \\
        &   & 4 & 1482.8307 & 1482.8344 & 5.5 & 8.6 & 9.8 & 1.3 & \\
        &   & 5 & 1482.9663 & 1482.9673 & 1.7 & 4.8 & 5.5 & 0.46 & \\
        &   & 6 & 1484.9602 & 1484.9648 & 7.2 & 2.0 & 2.4 & 0.59 & \\
        &   & 7 & 1485.8273 & 1485.8388 & 17.1 & 4.2 & 5.2 & 5.7 & \\
        &   & 8 & 1485.8874 & 1485.8886 & 2.2 & 1.1 & 1.7 & 0.12 & \\
        &   & 9 & 1485.9476 & 1485.9487 & 2.2 & 1.8 & 2.0 & 0.27 & \\
        &   & 10 & 1486.9588 & 1486.9619 & 5.0 & 1.9 & 2.8 & 0.39 & \\
        \hline
        & & & Cycle 3  & & & & & & \\
        \hline
        & 6 & 1 & 2190.0381 & 2190.0547 & 24.1 & 20.0 & 25.5 & 26.7 & 27.5 \\
        & & 2 & 2190.4401 & 2190.4409 & 1.7 & 1.9 & 2.3 & 0.27 & \\
        & & 3 & 2190.5027 & 2190.5038 & 1.7 & 3.5 & 3.7 & 0.37 &  \\
        & & 4 & 2190.5099 & 2190.5103 & 1.1 & 2.8 & 2.2 & 0.21 & \\
        & & 5 & 2190.9098 & 2190.9125 & 4.1 & 3.2 & 3.9 & 1.5 & \\
        & & 6 & 2191.1105 & 2191.1108 & 0.55 & 2.7 & 2.6 & 0.12 &  \\
        \hline
      AU Mic & 5 & 1 & 1340.7517 & 1340.7540 & 3.5 & 18.4 & 1.6 & 1.7 & 28.7 \\
             & & 2 & 1341.8232 & 1341.8249 & 2.8 & 23.5 & 2.2 & 3.5 & \\
             & & 3 & 1343.1545 & 1343.1556 & 2.2 & 13.0 & 1.5 & 2.4 & \\
             & & 4 & 1347.1380 & 1347.1421 & 6.1 & 19.7 & 1.6 & 6.8 & \\
             & & 5 & 1347.2673 & 1347.2767 & 13.6 & 35.5 & 2.9 & 45.5 &  \\
             \hline
             & & & Cycle 3 &  & & & & & \\
             \hline
             &1 & 1 & 2058.2364 &  & $>$9.6 & 99.2 & 7.0 & $>$96 & 28.8 \\
             
    %\hline
      %AX Mic &  & & No & Data & & & & &  \\
     \hline
      DG CVn & 3 &    1 & 1953.3826 & 1953.3835 & 1.5 & 11.2 & 6.9 & 3.9 & 28.4 \\
             & &    2 & 1953.4511 & 1953.4536 & 3.9 & 6.4 & 3.9 & 8.7 & \\
             & &    3 & 1953.7063 & 1953.7071 & 1.3 & 4.2 & 2.7 & 1.3 & \\
    \hline
      DX Cnc & 0 &    & & & & & & & 27.1 \\
      \hline
      EV Lac & 9 &  1  &  1748.0401 &  1748.0408 & 1.1 & 14.0 & 2.5 &  0.40 & 27.9 \\
             & & 2 &  1748.2379 & & $>$9.8 & 41.3 & 7.3 & $>$8.4 & \\
             & & 3 & 1749.0260 &  1749.0314 & 7.9 & 31.1 & 4.9 & 3.4 & \\
             & & 4&  1749.1059 & 1749.1075 & 2.4 & 15.0 & 2.4 & 0.57 & \\
             & & 5 &  1749.1663 & 1749.1669 & 0.92 & 60.2 & 9.6 & 1.4 & \\
             & & 6 & 1749.2232 &  1749.2238 & 1.1 & 19.1 & 2.8 & 0.48 & \\
             & & 7 &  1749.2952 & & $>$1.5 & 339.3 & 41.8 & $>$13.3 & \\
             & & 8$^{*}$ & & 1750.2256 & $>$11.4 & 20.9 & 3.1 & $>$3.4  & \\
             & & 9$^{*}$ & 1750.2913 &  1750.2917 & 0.74 & 14.2 & 2.1 & 0.22 & \\
      \hline
      %EZ AQr & &    & & & & & & & \\
      %\hline
      Fomalhaut C & 8 & 1 & 1361.8200 & 1361.8216 & 2.8 & 1.1 & 2.1 & 0.08 & 27.0 \\
                  & & 2 & 1361.8223 & 1361.8239 & 2.8 & 1.1 & 3.1 & 0.14 & \\
                  & &  3 & 1362.5573 & 1362.5584 & 1.8 & 2.1 & 7.2 & 0.24 &  \\
                  & & 4 & 1363.5597 & 1363.5603 & 1.1 & 3.1 & 9.5 & 0.21 & \\
                  & & 5 & 1364.7419 & 1364.7442 & 3.9 & 1.0 & 3.3 & 0.31 & \\
                  & & 6 & 1366.5982 & 1366.6007 & 3.9 & 5.7 & 14.5 & 0.83 & \\
                  & & 7 & 1366.6013 & 1366.6066 & 7.9 & 3.4 & 3.7 & 0.51 & \\
                  & & 8 & 1366.7375 & 1366.7387 & 1.8 & 2.1 & 5.3 & 0.16 & \\
    \hline
      %GJ 1061 & 0 & & No detection & & & & & & \\
    %\hline
      GJ 1284 & 1 &1 & 1381.4844 & 1381.4870 & 3.9 & 6.8 & 4.5 & 4.3 & 28.3 \\
      \hline
      %GJ 205 & & & Data unavailable & & & & & & \\
      %\hline
      %GJ 4353 & 0 & & No detection  & & & & & & \\
      %\hline
      GJ 832 & 0 & & & & & & & & 26.9 \\
      \hline
      Gliese 1 & 0 & & & & & & & & 26.7 \\
      \hline 
      Gliese 876 & 0 & & & & & & & & 26.3 \\
      \hline
      HIP 17695 & 2 &1 &1458.7890 & 1458.7916 & 3.9 & 3.9 & 3.4 & 3.7 & 28.3 \\
                & & 2 & 1461.1762 & 1461.1765 & 0.55 & 3.1 & 3.1 & 0.68  & \\
      \hline
      %HIP 23309 & & & Data unavailable & & & & & & \\
%\hline
      Kapteyn's Star & 0 & & & & & & & & 26.5 \\
      \hline
      Lacaille 9352 & 1 & 1 & 1365.2023 & 1365.2056 & 5.0 & 15.3 & 4.2 & 0.43 & 27.3 \\
      \hline
      %LHS 292 & 0 & & No detection & & & & & &  \\
      %\hline
      LP 776-25 & 3 & 1 & 1456.9436 & 1456.9449 & 2.0 & 8.4 & 7.3 & 2.3 & 28.2 \\
                & & 2 & 1461.8401 & 1461.8435 & 5.2 & 13.2 & 7.2 & 8.4 & \\
                & & 3 & & & $>$5.7 & $>$13.6 & $>$7.4 & $>$23.5 & \\
      \hline
      Luyten's Star & 1 & 1 & 1513.7822 & 1513.7868 & 7.2 & 0.9 & 4.1 & 0.07 & 26.5 \\
      \hline
      %NLTT 31625 & & & & & & & & & \\
      %\hline
      Prox. Cen. & 20 & & UVW1 Filter & & & & & & \\ 
      \hline
                & & 1$^{*}$ & 1584.2590 & 1584.2617 & 4.4 & 13.7 & 1.5 & 0.028 & 26.6 \\
                & & 2$^{*}$ & 1584.2660 & 1584.2669 & 1.5 & 17.4 & 2.2 & 0.016 & \\
                & & 3$^{*}$ & 1598.3523 & 1598.3537 & 2.2 & 16.3 & 2.2 & 0.022 & \\
                 & & 4 & 1604.3186 & 1604.3196 & 1.7 & 18.8 & 2.3 & 0.18 & \\
                 & & 5 & 1620.2601 & 1620.2613 & 2.2 & 20.8 & 1.5 & 0.015 & \\
                 & & 6 & 1620.3258 & 1620.3259 & 0.4 & 14.5 & 1.6 & 0.005 & \\
                 & & 7 & 1620.3287 & 1620.3306 & 3.3 & 16.3 & 1.8 & 0.025 & \\
                 \hline
                 & & & UVM2 filter& & & & & & \\
                 \hline
                 & & 1 & 1601.7311 & 1601.7314 & 0.55 & 4.8 & 5.3 & 0.006 & 26.0 \\
                 & & 2 & 1601.8003 & 1601.8007 & 0.74 & 3.1 & 3.6 & 0.007 & \\
                 & & 3 & 1602.6023 & 1602.6029 & 1.1 & 2.6 & 2.7 & 0.005 & \\
                 & & 4 & 1602.7232 & 1602.7239 & 1.3 & 59.7 & 49.7 & 0.061 & \\
                 & & 5 & 1602.7909 & 1602.7919 & 1.7 & 12.3 & 9.0 & 0.013 & \\
                 & & 6 & 1605.5754 & 1605.5760 & 1.1 & 5.5 & 4.4 & 0.008 & \\
                 & & 7 & 1605.6447 & 1605.6450 & 0.55 & 4.3 & 2.2 & 0.004 & \\
                 & & 8 & 1610.8212 & 1610.8225 & 2.0 & 4.6 & 3.3 & 0.009 & \\
                 & & 9$^{*}$ & 1652.8675 & 1652.8719 & 6.4 & 6.8 & 5.3 & 0.040 & \\
                 & & 10$^{*}$ & 1652.9252 & 1652.9282 & 4.4 & 13.2 & 9.4 & 0.061 & \\
                 & & 11$^{*}$ & 1659.6941 & 1659.6946 & 0.9 & 6.1 & 4.0 & 0.005 & \\
                 & & 12$^{*}$ & 1659.6957 & 1659.7026 & 10.1 & 11.1 & 9.4 & 0.12 & \\
                 & & 13$^{*}$ &  & 1665.5344 & $>$2.4 & 12.7 & 8.5 & $>$0.040 & \\
            \hline
      Ross 614 & 22 & 1 & 1472.9496 & 1472.9536 & 5.9 & 30.3 & 16.9 & 1.1 & 27.1 \\
                & & 2  & 1473.0121 & 1473.0126 & 0.92& 8.4 & 4.7& 0.085 & \\
                & & 3$^{*}$ & 1477.0694 &1477.0726 & 4.8 & 6.4  & 4.7 & 0.34 & \\
                & & 4$^{*}$ & 1477.0771 & 1477.0777 & 1.1 & 2.8 & 2.1 & 0.05 & \\
                & & 5$^{*}$ & 1477.2653 & 1477.2681 & 4.2 & 17.0 & 12.4& 0.92 & \\
                & & 6$^{*}$ & 1477.9891 & 1477.9915 & 3.7 & 5.4 & 3.8 & 0.31 & \\
                & & 7 & 1479.0510 & 1479.0581 & 10.3 & 35.6 & 20.7 & 1.2 & \\
                & & 8 & 1479.1241 & 1479.1243 & 0.55 & 5.2 & 3.0 & 0.05 & \\
                & & 9 & 1479.9115 & 1479.9195 & 11.8 & 11.4 & 7.1 & 1.2 & \\
                & & 10 & 1479.9762 & 1479.9765 & 0.55 & 3.9 & 2.4 & 0.03 & \\
                & & 11  & 1479.9832 & 1479.9908 & 11.0 & 30.7 & 19.2 & 2.5 & \\
                & & 12 & 1482.3105 & 1482.3111 & 1.1 & 3.7 & 2.6 & 0.07 & \\
                & & 13 &1483.0383  & 1483.0386 & 0.55 & 14.4 & 2.4 & 0.05 & \\
                & & 14  & 1483.0392 & 1483.0403 & 1.7 & 14.4 & 8.4 & 0.25 & \\
                & & 15 & 1483.0456 & 1483.0465 & 1.5 & 6.1 & 3.6 & 0.10 & \\
                & & 16 & 1483.0953 & 1483.0970 & 2.6 & 5.7 & 2.1 & 0.11  & \\
                & & 17 & 1483.0984 & 1483.0991 & 1.3 & 21.6 & 7.9 & 0.23 & \\
                & & 18 & 1483.1002 & 1483.1022 & 3.1 & 6.3 & 2.3 & 0.18 & \\
                & & 19 & 1483.9038 & 1483.9052 & 2.2 & 3.9 & 2.6 & 0.15 & \\
                & & 20 & 1483.9083 & 1483.9089 & 1.1 & 7.1 & 4.7& 0.14 & \\
                & & 21 & 1483.9587 & 1483.9611 & 3.7 & 3.8 & 2.5 & 0.18 & \\
                & & 22 & 1484.0268 & 1484.0281 & 2.0 & 3.5 & 2.4 & 0.07 & \\
      \hline
      TWa 22 & 6 & 1 &1551.9795 & 1551.9837 & 6.6 & 3.5 & 2.8 & 2.4 & 27.8 \\
            & & 2 & 1552.1094 & 1552.1117 & 3.9 & 1.5 & 2.0 & 0.87 & \\
            & & 3 & 1553.0385 & 1553.0402 & 2.6 & 2.7 & 6.6 & 1.7 & \\
            & & 4 & 1554.9663 & 1554.9686 & 3.9 & 1.1 & 2.6 & 1.3 & \\
            & & 5 & 1557.7611 & 1557.7631 & 3.3 & 1.1 & 2.9 & 1.6 & \\
            & & 6 & 1558.8177 & 1558.8183 & 1.1 & 1.3 & 3.7 & 0.59 & \\
       \hline     
      UV Ceti & & & & & & & & & \\
      \hline
      V1005 Ori & 4 & 1 & 1448.8960 & 1448.8999 & 5.9 & 17.3 & 5.4 & 38.2 & 29.0 \\
                & & 2 & 1450.5578 & 1450.5609 & 4.6 & 11.3 & 4.0 & 25.6 & \\
                & & 3 & 1455.0022 & 1455.0024 & 0.55 & 8.4 & 2.5 & 2.0 & \\
                & & 4 & 1455.0027 & 1455.0036 & 1.5 & 6.6 & 2.0 & 4.6 & \\
    \hline
      Wolf 359 & 15 & 1 & 3075.1950 & 3075.1953 & 0.74 & 5.8 & 3.3 & 0.006 & 26.10 \\
                & & 2 & 3075.1981 & 3075.1987 & 0.92 & 5.4 & 3.7 & 0.008 & \\
                & & 3 & 3095.6563 & 3095.6573 & 1.7 & 5.1 & 7.8 & 0.04 & \\
                &  & 4 & 3095.7215 & 3095.7227 & 2.0 & 3.0 & 9.2 & 0.03 & \\
                & & 5 & 3096.6433 & 3096.6446 & 2.0 & 22.3 & 53.2 & 0.16 & \\
                & & 6 &  3096.7180 & 3096.7184 & 0.74 & 1.8 & 6.4 & 0.02 & \\
                & & 7 & 3096.7695 & 3096.7731 & 5.3 & 4.6 & 3.8 & 0.04 & \\
                & & 8 & 3116.5682 & 3116.5702 & 3.3 & 1.4 & 2.9 & 0.03 & \\
                & & 9 & 3116.8306 & 3116.8373 & 9.8 & 13.7 & 25.7 & 0.41 & \\
                & & 10 & 3117.6946 & 3117.6949 & 0.55 & 2.0 & 4.4 & 0.009 & \\
                & & 11 & 3117.6963 & 3117.6969 & 1.10 & 2.0 & 6.5 & 0.02 & \\
                &  & 12 & 3118.0430 & 3118.0435 & 0.92 & 2.8 & 5.8 & 0.02 & \\
                & & 13 & 3118.0461 & 3118.0470 & 1.5 & 3.8 & 7.8 & 0.03 & \\
                & & 14 & 3118.1099 & 3118.1106 & 1.10 & 1.7 & 3.4 & 0.007 & \\
                & & 15 & 3118.8221 & 3118.8229 & 1.3 & 5.1 & 11.9 & 0.03 & \\
        \hline
                & & & Cycle 4 & & & & & & \\
        \hline
                & 33 & 1$^{*}$ & 2566.6048 & 2566.6056 & 1.3 & 1.7& 8.8 & 0.023 & 26.10 \\
                & & 2$^{*}$ & 2566.6061 & 2566.6075 & 2.2 & 20.1 & 51.8 & 0.13 & \\
                & & 3 & 2567.0573 & 2567.0579 & 1.1 & 1.6 & 5.0 & 0.014 & \\
                & & 4 & 2567.1946 & 2567.1948 & 0.55 & 1.2 & 3.1 & 0.006 & \\
                & & 5 & 2567.4039 & 2567.4063 & 3.7 & 40.9 & 70.2 & 0.21 & \\
                & & 6 & 2569.3817 & 2569.3823 & 1.1 & 2.6 & 6.4 & 0.017 & \\ 
                & & 7 & 2569.0498 & 2569.0514 & 2.8 & 1.6 & 3.7 & 0.030 & \\
                & & 8 & 2568.9305 & 2568.9313 & 1.3 & 4.7 & 10.6 & 0.025 & \\
                & & 9 & 2568.7330 & 2568.7336 & 0.92 & 4.9 & 6.5 & 0.015 & \\
                & & 10 & 2568.4603 & 2568.4605 & 0.55 & 1.7 & 5.3 & 0.010 & \\
                & & 11 & 2568.3906 & 2568.3913 & 1.3 & 4.1 & 10.7 & 0.044 & \\
                & & 12 & & 2568.1949 & $>$2.6 & 7.0 & 8.2 & $>$0.032 & \\
                & & 13 & 2568.1967 & 2568.1969 & 0.55 & 3.0 & 3.5 & 0.005 & \\
                & & 14 &  & 2569.0006 & $>$17.1 & 9.9 & 24.6 & $>$1.5 & \\
                & & 15 & 2570.3258 & 2570.3279 & 3.1 & 25.5 & 53.0 & 0.22 & \\
                & & 16 & 2570.2368 & 2570.2373 & 0.92 & 2.4 & 2.9 & 0.007 & \\
                & & 17 & 2570.2457 & 2570.2461 & 0.74 & 6.8 & 8.0 & 0.014 & \\
                & & 18 & 2570.1765 & 2570.1773 & 1.5 & 2.2 & 6.4 & 0.021 & \\
                & & 19 & 2570.1072 & 2570.1082 & 1.7 & 5.1 & 11.8 & 0.038 & \\
                & & 20 & 2569.9221 & 2569.9230 & 1.5 & 4.1 & 12.3 & 0.037 & \\
                & & 21 & 2569.8556 & 2569.8564 & 1.3 & 2.7 & 7.0 & 0.021 & \\
                & & 22 & 2569.7939 & 2569.7943 & 0.74 & 1.4 & 5.1 & 0.013 & \\
                & & 23 & 2569.5880 & 2569.5882 & 0.55 & 2.5 & 6.0 & 0.012 & \\
                & & 24 & 2569.5886 & 2569.5909 & 3.5 & 6.4 & 15.8 & 0.060 & \\
                & & 25 & 2570.5064 & 2570.5070 & 1.1 & 2.5 & 6.3 & 0.027 & \\
                & & 26 & 2570.5758 & 2570.5772 & 2.2 & 2.6 & 6.7 & 0.033 & \\
                & & 27 & 2570.9173 & 2570.9177 & 0.74 & 3.0 & 7.7 & 0.013 & \\
                & & 28 & 2570.9198 & 2570.9203 & 0.92 & 1.9 & 4.8 & 0.014 & \\
                & & 29 & 2571.0525 & 2571.0529 & 0.74 & 1.2 & 4.2 & 0.012 & \\
                & & 30 & 2571.1166 & 2571.1209 & 6.4 & 26.2 & 31.3 & 0.17 & \\
                & & 31 & 2571.2359 & 2571.2363 & 0.74 & 3.0 & 2.9 & 0.004 & \\
                & & 32 & 2571.8443 & 2571.8454 & 1.8 & 1.6 & 4.6 & 0.014 & \\
                & & 33 & 2572.0482 & 2572.0497 & 2.4 & 3.4 & 8.9 & 0.057 & \\
                
        \hline
      Wolf 424 & 5 & 1 & 1948.2044 & 1948.2053 & 1.5 & 4.5 & 3.3 & 0.082 & 27.1 \\
                & & 2 & 1948.7302 &  & $>$1.3 & 5.8 & 6.1 & $>$0.23 & \\
                & & 3 & 1949.3953 & 1949.3990 & 5.5 & 34.0 & 35.1 & 1.5 & \\
                & & 4 & 1949.5879 & 1949.5882 & 0.55 & 3.4 & 3.2 & 0.060 & \\
                & & 5 & 1949.5959 & 1949.5964 & 0.92 & 3.8 & 3.5 & 0.087 & \\
         %\hline       
      %WX UMa & 0 & & & & & & & & 26.4\\
      \hline
      YZ Ceti & 11 & 1 & 1401.6173 & 1401.6194 & 3.1 & 7.5 & 21.3 & 0.13 & 26.2 \\
             & & 2 & & 1402.2084 & $>$6.1 & 3.0 & 8.1 & $>$0.16 &  \\
             & & 3 & 1402.5384 & 1402.5407 & 3.5 & 2.3 & 10.6 & 0.11 & \\
             & & 4 & 1403.9915 & 1403.9924 & 1.5 & 1.1 & 4.8 & 0.019 & \\
             & & 5 & 1404.0674 & 1404.0682 & 1.3 & 1.1 & 4.8 & 0.024 & \\
             & & 6 & 1404.1342 & 1404.1349 & 1.3 & 2.0 & 8.2 & 0.023 & \\
             & & 7 & 1404.1360 &  & $>$0.74 & 2.0 & 8.4 & $>$0.032 & \\
             & & 8 & 1404.6538 & 1404.6559 & 3.1 & 7.1 & 21.9 & 0.11 & \\
             &  & 9 & 1404.6662 & 1404.6675 & 2.0 & 6.1 & 18.6 & 0.17 & \\
             & & 10 & 1404.7819 & 1404.7824 & 0.92 & 1.7 & 5.1 & 0.016 & \\
             &  & 11$^{*}$ & 1407.6387 & 1407.6393 & 1.1 & 4.7 & 22.3 & 0.064 & \\
     \hline
      YZ CMi & 21 & 1 & 1508.5441 & 1508.5475 & 5.2 & 17.6 & 3.9 & 2.3 & 27.9 \\
             & & 2 & & 1508.6844 & $>$24.3 & 60.4 & 13.5 & $>$62.8 & \\
             & & 3 & 1509.5400 & 1509.5479 & 11.6 & 23.3 & 4.7 & 4.2 & \\
             & & 4 & 1509.5502 & 1509.5506 & 0.74 & 10.4 & 2.1 & 0.15 & \\
             & & 5 & 1509.5534 & 1509.5543 & 1.5 & 10.4 & 2.0 & 0.42 & \\
             & & 6 & 1509.5946 & 1509.5987 & 6.1 & 24.7 & 5.0 & 3.3 & \\
             & & 7 & 1509.6074 & 1509.6082 & 1.3 & 9.4 & 1.9 & 0.19 & \\
             & & 8 & 1509.6636 & 1509.6645 & 1.5 & 14.5 & 2.9 & 0.26 & \\
             & & 9 & 1510.5425 & 1510.5432 & 1.3 & 9.1 & 2.3 & 0.25 & \\
             & & 10 & 1511.7955 & 1511.7974 & 3.3 & 6.5 & 1.7 & 0.66 & \\
             & & 11 & 1511.8031 & 1511.8039 & 1.7 & 5.6 & 1.5 & 0.19 & \\
             & & 12 & 1513.1850 & 1513.1927 & 11.2 & 74.5 & 19.2 & 10.7 & \\
             & & 13 & 1513.3260 & 1513.3267 & 1.10 & 8.2 & 2.1 & 0.26 & \\
             & & 14 & 1514.3858 & 1514.3871 & 2.0 & 9.8 & 2.3 & 0.64 & \\
             & & 15 & 1514.9865 & 1514.9881 & 2.6 & 20.8 & 5.8 & 2.0 & \\
             & & 16 & 1514.9883 & 1514.9911 & 4.2 & 20.8 & 3.0 & 1.7 & \\
             & & 17 & 1515.0552 & 1515.0564 & 2.0 & 22.6 & 6.4 & 1.1 & \\
             & & 18 & 1515.0599 & 1515.0628 & 4.4 & 12.3 & 2.2 & 1.0 & \\
             & & 19$^{*}$ &  1516.1752 & 1516.1756 & 0.74 & 12.6 & 2.3 & 0.19 & \\
             & & 20$^{*}$ & 1516.3020 & 1516.3067 & 7.0 & 15.4 & 2.9 & 2.3 & \\
             & & 21$^{*}$ & 1516.3145 & 1516.3167 & 3.3 & 15.4 & 2.1 & 0.76 & \\
             \hline
             & & & Cycle 3 & & & & & & \\
             \hline
             & 10 & 1 & 2236.9036 & 2236.9162 & 18.4 & 83.5 & 26.6 & 29.1 & 27.8 \\
             & & 2 & 2236.9712 & 2236.9725 & 2.0 & 7.1 & 2.3 & 0.41 & \\
             &  & 3 & 2237.0412 & 2237.0467 & 8.1 & 28.8 & 9.2 & 4.1 & \\
             & & 4 & 2237.0542 & & $>$0.55 & 7.7 & 2.5 & $>$0.18 & \\
             & & 5 & 2237.7000 & 2237.7007 & 1.3 & 47.7 & 4.8 & 0.60 & \\
             & & 6 & 2237.7061 &  & $>$9.2 & 41.6 & 4.2 & $>$6.4 & \\
             & & 7 & 2237.7658 & 2237.7662 & 0.74 & 15.8 & 2.6 & 0.28 & \\
             & & 8 & 2237.7671 & 2237.7675 & 0.74 & 21.1 & 3.3 & 0.32 & \\
             & & 9 & 2237.7801 & 2237.7815 & 2.2 & 41.0 & 6.5 & 2.0 & \\
             & & 10 & 2238.0325 & 2238.0339 & 2.2 & 10.5 & 5.8 & 1.5 & \\
             \hline
GJ 3631 & 16 & 1$^{*}$ & 2552.2628 & 2552.2643 & 2.8 & 1.1 & 4.0 & 0.21 & 26.9 \\ 
              & & 2$^{*}$ & 2552.4681 & 2552.4685 & 0.74 & 1.2 & 10.9 & 0.15 & \\
              & & 3 & 2556.2342 & 2556.2352 & 1.7 & 3.6 & 14.3 & 0.18 & \\
              & & 4 & 2559.3030 & 2559.3035 & 0.92 & 1.5 & 8.2 & 0.11 & \\
              & & 5 & 2561.0782 & 2561.0785 & 0.55 & 1.9 & 4.8 & 0.062 &  \\
              & & 6 & 2563.2749 & 2563.2908 & 23.0 & 6.9 & 63.1 & 16.9 & \\
              & & 7 & 2563.8788 & 2563.8798 & 1.7 & 2.2 & 6.9 & 0.17 &  \\
              & & 8 & 2564.4070 & 2564.4079 & 1.5 & 2.5 & 14.4 & 0.40 & \\
              & & 9 & 2564.4197 & 2564.4200 & 0.55 & 1.1 & 8.3 & 0.12 & \\
              & & 10 & 2568.7818 & 2568.7823 & 0.92 & 5.4 & 71.5 & 1.1 & \\
              & & 11 & 2568.1261 & 2568.1278 & 2.6 & 3.3 & 11.6 & 0.31 & \\
              & & 12 & 2570.7771 & 2570.7772 & 0.37 & 2.2 & 23.0 & 0.25 & \\
              & & 13 & 2575.6136 & 2575.6157 & 3.1 & 5.4 & 17.9 & 0.40 & \\
              & & 14 & 2575.6255 & 2575.6272 & 2.6 & 5.3 & 16.9 & 0.37 & \\
              & & 15 & 2576.4823 & 2576.4826 & 0.55 & 1.1 & 14.7 & 0.19 & \\
              & & 16 & 2576.4831 & 2576.4834 & 0.74 & 0.8 & 10.2 & 0.18 
    \label{table:UV flare properties}
              
\end{longtable}

%%%%%%%%%%%%%%%%%
%TESS FLARES OBSERVED SIMULTANEOULSY WITH Swift/UVOT
%%%%%%%%%%%%%%%%%%%

\begin{longtable}{|l|l|l|l|l|l|l|l|l|}
\caption{Summary of TESS/K2 flare properties} \label{tab:tess_flares} \\

\hline \multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{$N_{U}$}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{$T_{\rm start}$}} & 
\multicolumn{1}{c|}{\textbf{$T_{\rm stop}$}} & \multicolumn{1}{c|}{$T_{\rm peak}$} & 
\multicolumn{1}{c|}{\textbf{ED}}  & \multicolumn{1}{c|}{\textbf{log $E$}} & \multicolumn{1}{c|}{\textbf{amplitude}}
\\
\hline  \multicolumn{1}{|c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{}}  & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & 
\multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & \multicolumn{1}{c|}{BJD - 2457000 (d)} & 
\multicolumn{1}{c|}{min}  & \multicolumn{1}{c|}{\textbf{erg}}  & \multicolumn{1}{c|}{} \\
\hline 
\endfirsthead

\multicolumn{9}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\hline \multicolumn{1}{|c|}{\textbf{Name}} & \multicolumn{1}{c|}{\textbf{$N_{U}$}} & \multicolumn{1}{c|}{\textbf{}} & \multicolumn{1}{c|}{\textbf{$T_{\rm start}$}} & 
\multicolumn{1}{c|}{\textbf{$T_{\rm stop}$}} & \multicolumn{1}{c|}{$T_{\rm peak}$} & 
\multicolumn{1}{c|}{\textbf{ED}}  & \multicolumn{1}{c|}{\textbf{log $E$}} & \multicolumn{1}{c|}{\textbf{amplitude}}  \\ \hline 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & 
\multicolumn{1}{c|}{\scriptsize{BJD - 2457000 (d)}} & \multicolumn{1}{c|}{BJD - 2457000 (d)} & 
\multicolumn{1}{c|}{min}  & \multicolumn{1}{c|}{erg}  & \multicolumn{1}{c|}{}] \\
\hline
\endhead

\hline \multicolumn{9}{|r|}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot
AP Col & & & 1473.08486&	1473.08763&	1473.08486&	1.8&	32.0&	1.008\\
&&& 1482.05429&	1482.05429&	1482.05429&	0.52&	31.5&	1.004 \\
&&& 1484.96121&	1484.96538&	1484.96121&	1.3&	31.9&	1.003\\
&&&2190.04074&	2190.05625&	2190.04074&	13.1&	32.9&	1.023\\
\hline
AU Mic & & & 2058.2366&	2058.29632&	2058.2366&	15.6&	34.0&	1.009 \\
\hline
EV Lac & && 1748.2384&	1748.2467&	1748.2384&	1.5&	31.8&	1.003\\
 & & & 1749.0273&	1749.0328&	1749.0286&	1.2&	31.7&	1.003	\\
 & & & 1749.2953&	1749.3036&	1749.2967&	4.8&	32.3&	1.013\\
\hline
GJ 3631&5&1&2561.07663&	2561.090527&	2561.076637&	0.75&	31.3&	1.01\\
&&2&2563.2758&	2563.2883&	2563.2758&	32.7&	32.9&	1.06\\
&&3&2563.87968&	2563.88524&	2563.87968&	0.45	&31.0&	1.01\\
&&4&2564.4214&	2564.43807&	2564.4214&	5.4&	32.1&	1.05\\
&&5&2568.12731&	2568.13008&	2568.12731&	0.63&	31.2&	1.01\\
\hline
LP 776-25 & & & 1456.94462&	1456.94601&	1456.94462&	0.60&	32.2&	1.003 \\
&&& 1461.84041&	1461.84874&	1461.84041&	2.6&	32.9&	1.006 \\
\hline
Prox. Cen. & & & 1602.72307&	1602.72307&	1602.72307&	0.16&	30.1&	1.001 \\
\hline
Ross 614 & 5&1 & 1472.94935&	1472.95213&	1472.95074&	0.88&	31.6&	1.004\\
&&2&1479.91469&	1479.91885&	1479.91469&	1.09&	31.7&	1.003 \\
&&3&1479.98413&	1479.99524&	1479.98413&	3.0&	32.1&	1.006 \\
&&4&1483.90914&	1483.91331&	1483.90914&	0.7236&	31.5&	1.002\\
&&5&1483.95775&	1483.95914&	1483.95775&	0.49&	31.3&	1.002\\
\hline
V1005 Ori & & & 1448.896787&	1448.896787&	1448.896787&	0.31&	32.6&	1.003\\
\hline
Wolf 359 & 6 & 1 & 2567.40392 & 2567.40647	& 2567.40392 &	1.4 &	30.9 &	1.02 \\
(TESS)& &2 & 2568.39059&	2568.39082&	2568.39059&	0.25&	30.2&	1.007 \\
&&&2568.98741&	2569.0057&	2568.98741&	11.5&	31.9&	1.012\\
&&3&2570.10743&	2570.10789&	2570.10743&	0.36&	30.4&	1.008 \\
& &4 &2570.32597&	2570.32805&	2570.32597&	1.3&	30.9&	1.018 \\
& & 5&2570.50654&	2570.50723&	2570.50654&	0.43&	30.4&	1.008 \\
& &6 &2571.11678&	2571.11864&	2571.11678&	1.2&	30.9&	1.013 \\
\hline
Wolf 359 &&1&3075.19455&	3075.19592&	3075.19455&	0.47&	29.6&	1.006 \\
($K$2)& & 2&3075.19728&	3075.20068&	3075.19728&	1.12&	29.95&	1.004 \\
& & 3&3095.656&	3095.66491&	3095.656&	1.31&	30.03&	1.005 \\
& & 4&3096.64361&	3096.64905&	3096.64361&	2.25&	30.26&	1.0239	\\
& & 5&3116.56805&	3116.57895&	3116.56805&	0.97&	29.89&	1.0023 \\
& & 6&3116.83094&	3116.84252&	3116.83094&	8.05&	30.81&	1.0200 \\
& & 7&3117.69657&	3117.69861&	3117.69657&	0.125&	29.00&	1.0012\\
& & 8&3118.04322&	3118.04322&	3118.04322&	0.06&	28.695&	1.0010\\
& & 9&3118.04595&	3118.04799&	3118.04595&	0.18&	29.16&	1.002 \\
& & 10&3118.10929&	3118.11269&	3118.10929&	0.21&	29.22&	1.001 \\
& & 11&3118.82235&	3118.82371&	3118.82235&	0.36&	29.46&	1.003 \\
\hline
Wolf 424 & & & 1949.3954&	1949.3968&	1949.3954&	0.52&	31.2&	1.002 \\
\hline
YZ CMi & & & 1508.65524&	1508.71219&	1508.65524&	122.6&	34.1&	1.132\\
&6&&1513.18573&	1513.19406&	1513.18573&	2.8&	32.4&	1.009\\
&&&1514.98985&	1514.99263&	1514.98985&	0.81&	31.9&	1.003\\
 & & & 2236.9053&	2236.90993&	2236.9053&	4.5	&32.6&	1.021\\
&&&2237.04165&	2237.0435&	2237.04165&	0.60&	31.8&	1.006\\
&&&2237.7002& 2237.70159&	2237.7002&	0.26&	31.4&	1.005\\
&&&2237.70622&	2237.71826&	2237.70622&	6.26&	32.8&	1.013\\
&&&2237.78053&	2237.78238&	2237.78053&	0.79&	31.9&	1.009
\label{table:tess flare properties}
              
\end{longtable}


% \end{document}
